Monitoring Data Minimisation

Data minimisation is a privacy enhancing principle, stating that personal data collected should be no more than necessary for the specific purpose consented by the user. Checking that a program satisfies the data minimisation principle is not easy, even for the simple case when considering deterministic programs-as-functions. In this paper we prove (im)possibility results concerning runtime monitoring of (non-)minimality for deterministic programs both when the program has one input source (monolithic) and for the more general case when inputs come from independent sources (distributed case). We propose monitoring mechanisms where a monitor observes the inputs and the outputs of a program, to detect violation of data minimisation policies. We show that monitorability of (non) minimality is decidable only for specific cases, and detection of satisfaction of different notions of minimality in undecidable in general. That said, we show that under certain conditions monitorability is decidable and we provide an algorithm and a bound to check such properties in a pre-deployment controlled environment, also being able to compute a minimiser for the given program. Finally, we provide a proof-of-concept implementation for both offline and online monitoring and apply that to some case studies.

==> content/monitorability.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Runtime monitoring Vs. using monitors for pre-deployment testing}
\label{sec:monitorability}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From the definitions of $M_{\varphi_m}$ (resp. $M_{\varphi_{sdm}}$) for monitoring monolithic (resp. distributed) minimality properties, providing conclusive verdict $\true$  from an observed input-output word $\sigma \in \Sigma^*$,
in addition to testing $\satMin(\sigma)$ (resp. $\satMinD(\sigma)$), the monitor has to be provided with information about the set of all possible inputs $I$, and we need to check whether every possible input appear in $\sigma$ at least once (i.e., test whether $\inpExh(I, \sigma)$ holds).

The discussion of this section applies to both the monolithic and distributed cases. To simplify presentation, the discussion considers monitoring of monolithic minimality.

\remove{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}
For any given word $\sigma \in \Sigma^*$ (where $\Sigma = I\times O$), testing whether every input belonging to $I$ appears in $\sigma$ at least once (i.e., testing $\inpExh(I, \sigma)$) is feasible in general iff the set of inputs $I$ and $\sigma$ are finite and bounded.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}

In runtime monitoring, the word $\sigma \in \Sigma^*$ (observation of current execution of $\calP$) that is fed to a monitor is of finite bounded length ($\sigma$ and its length are both known).  Thus, for any given $\sigma\in \Sigma^*$ and any set of inputs $I$, testing $\inpExh(I, \sigma)$ is straightforward, as illustrated in
Algorithm \ref{algo:inpExt}.
%for testing $\inpExh$ for any given $\sigma \in \Sigma^*$ and any given $I$ is illustrated below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[ht]
	\caption{$ \inpExh(I, \sigma) $}
	\label{algo:inpExt}
	{
		\begin{algorithmic}[1]
			\STATE $I' \gets \{ \} $
			\FOR{$ i \in [ |1, |\sigma| ] $}
			\STATE $inp \gets \Pi_1(\sigma_i)$
			\STATE $I' \gets I' \cup \{ inp \}$
			\IF{$|I'| = |I|$}
			\RETURN $\true$
			\ENDIF		
		%	\STATE $I' \gets I' \setminus \{i\}$
			\ENDFOR
			\RETURN $\false$
		\end{algorithmic}
	}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Algorithm \ref{algo:inpExt}, requires the set of possible inputs $I$, and an input-output word $\sigma \in \Sigma^*$ (where $\Sigma = I\times O$) as input parameters. $I'$ which is initially empty is used to keep track of the set of inputs seen in $\sigma$.
While processing the sequence $\sigma$ event by event to build $I'$, if
$|I'| = |I|$, then the algorithm returns $\true$ and terminates.
In the worst-case, the for-loop runs for $|\sigma|$ times.  After processing all the events in $\sigma$, if $|I'| \neq |I|$ then the algorithm returns $\false$.

Note that one simple check before entering the for-loop in Algorithm  \ref{algo:inpExt} is to check if $|\sigma| < |I|$. In this case, we can immediately return $\false$ if $|\sigma| < |I|$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}[When $|\sigma| < |I|$]
	\label{prop:inpLength}
	When the length of the input-output word $\sigma \in \Sigma^*$
	is less that the cardinality of the set of inputs, then $\inpExh(I, \sigma)$ is $\false$.
	\[\forall \sigma\in \Sigma^*: |\sigma| < |I| \implies \inpExh(I, \sigma) = \false\].
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{remark}[Conclusive verdict $\true$ during runtime monitoring]
In general, when we consider monitoring inputs and outputs of program $\calP$ (resp. $\calDP$) at runtime, and providing knowledge of the set of all possible inputs to the monitor,  where $\sigma \in \Sigma^*$ is the current observation of execution of $\calP$ (resp. $\calDP$), it is highly unlikely that $\sigma$ covers all the inputs in $I$. Thus, as we can imaging, during runtime monitoring
$ \inpExh(I, \sigma)$ most likely will return $\false$, and thus the condition of the first case (that provides conclusive verdict $\true$) in Definition \ref{def:monitor:mono2} (resp. Definition  \ref{def:monitor:dist}) can be hardly seen in practice.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\remove{
\begin{remark}[Monitor $M$ (resp. $M_{dm}$ with two cases]
	If we notice the condition for the first case (i.e, in order to provide conclusive verdict $\true$), checking whether $\satMin$ (resp. $\satMinD$) holds for the current observation $\sigma$ is not sufficient, and we also need to check  $\satMin$ (resp. $\satMinD$) for any possible extension of $\sigma$.
	Thus, in general, it is not possible to check condition of the first case, from an observed execution $\sigma$ of $\calP$ (resp. $\calDP$).
	We thus consider checking only the condition of the second case, i.e., checking whether $\satNonMin$ (resp. $\satNonMinD$) holds for the current observation $\sigma$ to provide conclusive verdict $\false$, and return unknown ($?$) if $\satNonMin$ (resp. $\satNonMinD$) returns $\false$ for $\sigma$.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}[]
For monitor $M$ (resp. $M_{dm}$), providing conclusive verdict $\true$, only from an observed input-output behavior $\sigma \in \Sigma^*$ that is observed execution of $\calP$ (resp. $\calDP$)  is not possible.	
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}[Providing conclusive verdict $\true$]
	\label{prop:min}
	For any current observation $\sigma\in\Sigma^*$ testing the condition of the first case of the monitor (which is $\satMin(\sigma) \wedge \forall \sigma'\in \Sigma^*: \sigma\pref \sigma', \satMin(\sigma')$) reduces to testing  whether  whether $\satMin(\sigma)$ holds iff the following condition holds for $\sigma$:
	
	\[\forall inp \in I, \exists id \in [1, |\sigma|]: \Pi_1(\sigma_{id}) = inp\].
	
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}

However, monitor $M_{\varphi_m}$ (resp. $M_{\varphi_{sdm}}$) can be used for testing for minimality prior to deployment. In this case, the input observation fed to the monitor can be generated in such a way that it covers all the inputs in $I$ (when $I$ is finite and bounded).

\subsection{Testing in a controlled environment via monitoring}
%For some observation $\sigma$, when does testing the condition of the first case  which is $\satMin(\sigma) \wedge \forall \sigma'\in \Sigma^*: \sigma\pref \sigma', \satMin(\sigma')$ reduce to testing whether $\satMin(\sigma)$ holds?
%We consider program $\calP$ to be repeated execution of function $\calF: I \rightarrow O$.
%
When the set of inputs $I$ is bounded, and when testing $\calP$ in a controlled environment (i.e., when we have control over the inputs that are fed to $\calP$), it is indeed possible to obtain a conclusive verdict (either $\true$ or $\false$), upon observing a sequence $\sigma$ of length $|I|$.
We discuss this further via the monolithic case, which straightforwardly extends to the distributed case.

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[ht]
	\caption{$\mathsf{DataMinTester- Program \calP}$}
	\label{algo:minTester}
	{
		\begin{algorithmic}[1]
			\STATE $I' \gets I$, $\sigma \gets \epsilon$, $v \gets ?$
			\WHILE {($|I'| > 0 \wedge v==?$)}
			\STATE $i \gets pickInp(I')$
			\STATE $o \gets \calF(i)$
			\STATE $\sigma \gets \sigma \cdot(i,o)$
			\STATE $v \gets M_\varphi(\sigma)$
			\STATE $I' \gets I' \setminus \{i\}$
			\ENDWHILE
		\end{algorithmic}
	}
\end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Algorithm for testing $\calF$ via monitoring is illustrated in Algorithm \ref{algo:minTester}.
%DataMinTester presented in this algorithm can be considered as program $\calP$ corresponding to $\calF$.
In Algorithm \ref{algo:minTester}, $I'$ contains inputs that are not yet fed to the function $\calF$.
Initially, $I'$ is assigned with the set of inputs $I$.
In every iteration of the while loop, an input $i$ from the set $I'$ is picked non-deterministically, which is fed to $\calF$, and $\calF(i)$ is assigned to $o$. The input-output event $(i,o)$ is then fed to the monitor.
Before proceeding to the next iteration, input $i$ which is already considered in the current iteration is removed from the set $I'$.

DataMinTester in Algorithm \ref{algo:minTester} can be considered as program $\calP$ where  function $\calF$ is executed repeatedly.
However, here, in every iteration we invoke $\calF$ with a new input from the set $I$ (i.e., input that has not been considered in the previous iterations).
The while loop thus terminates after $|I|$ iterations.


After $|I|$ iterations of the algorithm, the input-output word $\sigma$ that the monitor receives will be of length $|I|$, and $\inpExh(I, \sigma)$ will evaluate to $\true$.
%
The monitor $M_{\varphi_m}$ certainly returns a conclusive verdict upon receiving an input-output word of length $|I|$.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}
Let $\sigma \in \Sigma^*$ be an execution of the $\mathsf{DataMinTester}$ in Algorithm \ref{algo:minTester}, which is a sequence of input-output word fed to the monitor.
The length of $\sigma$ will be at most $|I|$, and
 the monitor will certainly return a conclusive verdict $\top$ or $\bot$ for  $\sigma$ of length $|I|$.
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%
Regarding conclusive verdict $true$ (i.e, about satisfaction of minimality),  the monitor cannot provide this verdict before observing a word of length $|I|$.
Regarding conclusive verdict $false$ (i.e, about violation of minimality),  the monitor may be able to provide this verdict before observing word of length $|I|$.
In this case, the execution of the tester program can stop earlier soon after the monitor observes the sequence that satisfies non-minimality property.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


==> content/pre-mon.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Pre-deployment testing and on monitorability of (non) minimality properties}
\label{sec:monitorability}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\red{to update this section!!}

From the definitions of monitors $M$ (resp. $M_{dm}$) for monitoring monolithic (resp. distributed) minimality properties, providing conclusive verdict $\true$  from observed input-output word $\sigma$ is no possible in general. From the condition tested in the first case of Definition \ref{def:monitor:mono} (resp. Definition \ref{def:monitor:dist}), we can notice that checking condition $\satMin$ (resp. $\satMinD$) for $\sigma$ is not sufficient, and this also has to be tested for every possible continuation of $\sigma$.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}[Monitor $M$ (resp. $M_{dm}$ with two cases]
	If we notice the condition for the first case (i.e, in order to provide conclusive verdict $\true$), checking whether $\satMin$ (resp. $\satMinD$) holds for the current observation $\sigma$ is not sufficient, and we also need to check  $\satMin$ (resp. $\satMinD$) for any possible extension of $\sigma$. 
	Thus, in general, it is not possible to check condition of the first case, from an observed execution $\sigma$ of $\calP$ (resp. $\calDP$).
	We thus consider checking only the condition of the second case, i.e., checking whether $\satNonMin$ (resp. $\satNonMinD$) holds for the current observation $\sigma$ to provide conclusive verdict $\false$, and return unknown ($?$) if $\satNonMin$ (resp. $\satNonMinD$) returns $\false$ for $\sigma$.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}[]
For monitor $M$ (resp. $M_{dm}$), providing conclusive verdict $\true$, only from an observed input-output behavior $\sigma \in \Sigma^*$ that is observed execution of $\calP$ (resp. $\calDP$)  is not possible.	
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}[Providing conclusive verdict $\true$]
	\label{prop:min}
	For any current observation $\sigma\in\Sigma^*$ testing the condition of the first case of the monitor (which is $\satMin(\sigma) \wedge \forall \sigma'\in \Sigma^*: \sigma\pref \sigma', \satMin(\sigma')$) reduces to testing  whether  whether $\satMin(\sigma)$ holds iff the following condition holds for $\sigma$:
	
	\[\forall inp \in I, \exists id \in [1, |\sigma|]: \Pi_1(\sigma_{id}) = inp\].
	
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Testing in a controlled environment via monitoring}
%For some observation $\sigma$, when does testing the condition of the first case  which is $\satMin(\sigma) \wedge \forall \sigma'\in \Sigma^*: \sigma\pref \sigma', \satMin(\sigma')$ reduce to testing whether $\satMin(\sigma)$ holds?
%We consider program $\calP$ to be repeated execution of function $\calF: I \rightarrow O$.
%
When the set of inputs $I$ is bounded, and when testing $\calP$ in a controlled environment (i.e., when we have control over the inputs that are fed to $\calP$), it is indeed possible to obtain a conclusive verdict (either $\true$ or $\false$), upon observing a sequence $\sigma$ of length $|I|$.  


%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[ht]
	\caption{$\mathsf{DataMinTester- Program \calP}$}
	\label{algo:enf}
	{
		\begin{algorithmic}[1]
			\STATE $I' \gets I
			$
			\WHILE {$|I'| > 0$}
			\STATE $i \gets rand(I')$
			\STATE $o \gets \calF(i)$
			\STATE $notifyMonitor((i,o))$
			\STATE $I' \gets I' \setminus \{i\}$
			\ENDWHILE
		\end{algorithmic}
	}
\end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

Algorithm for testing $\calF$ via monitoring is illustrated in Algorithm \ref{algo:enf}. 
%DataMinTester presented in this algorithm can be considered as program $\calP$ corresponding to $\calF$.
In Algorithm \ref{algo:enf}, $I'$ contains inputs that are not yet fed to the function $\calF$. 
Initially, $I'$ is assigned with the set of inputs $I$.
In every iteration of the while loop, an input $i$ from the set $I'$ is selected randomly, which is fed to $\calF$, and $\calF(i)$ is assigned to $o$. The input-output event $(i,o)$ is then fed to the monitor. 
Before proceeding to the next iteration, input $i$ which is already considered in the current iteration is removed from the set $I'$.
  
DataMinTester in Algorithm \ref{algo:enf} can be considered as program $\calP$ where  function $\calF$ is executed repeatedly. 
However, here, in every iteration we invoke $\calF$ with a new input from the set $I$ (i.e., input that has not been considered in the previous iterations). 
The while loop thus terminates after $|I|$ iterations. 


After $|I|$ iterations of the algorithm, the input-output word $\sigma$ that the monitor receives will be of length $|I|$, and it will satisfy the condition in Proposition \ref{prop:min}.
%
The monitor should certainly return a conclusive verdict upon receiving a input-output word of length $|I|$.


Regarding conclusive verdict $true$ (i.e, about satisfaction of minimality),  the monitor cannot provide this verdict before observing word of length $|I|$.
Regarding conclusive verdict $false$ (i.e, about violation of minimality),  the monitor may be able to provide this verdict before observing word of length $|I|$.
In this case, the execution of the tester program can stop earlier soon after the monitor observes the sequence that satisfies non-minimality property. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Monitorability}
\red{TODO!}


A monitor takes a word $\sigma\in \Sigma^*$ (observation of current execution of program $\calP$) and it emits verdicts.\red{Introduce and mention about three valued semantics from RV, where true and false are conclusive verdicts}.  

Given property $\varphi \subseteq \Sigma^*$,  a monitor $M$ for property $\varphi$ should satisfy the following constraints:

\begin{itemize}
	\item For any observation $\sigma\in \Sigma^*$,  if the monitor provides a conclusive verdict  true (resp. false) for $\sigma$, 
	then $\sigma$ followed by any extension $\sigma' \in \Sigma^*$ of $\sigma$ (i.e., $ \sigma \pref \sigma'$) satisfies (resp. violates) property $\varphi$.
	%
	\item The monitor should provide a conclusive verdict as soon as possible. 
	For any $\sigma \in \Sigma^*$, if the verdict given by a monitor is inconclusive for $\sigma$, then for any prefix $\sigma'$ of $\sigma$ (i.e., $ \sigma' \pref \sigma$), the property that we want to verify does not hold for $\sigma'$.
\end{itemize}	


%%%%%%%%%%%%%%%%%%%%%%%%%

\red{What is non-monitorability in our context/for our problem?}

\red{We can perhaps say that a property $\varphi \subseteq \Sigma^*$ is monitorable if there exists a monitor $M$ for $\varphi$, and if there exists a word of finite length $\sigma \in \Sigma^*$, where the monitor $M$ can give a conclusive verdict for $\sigma$.}

\remove{
\red{
3. When is a Property P monitorable?
%
A Property P is monitorable if there exists a finite word $\sigma$ (we can perhaps give some bound on the length), and if there exists a best monitor that returns a conclusive verdict for $\sigma$.
}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Monitorbility of Property $\varphi$.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}
A property $\varphi \subseteq \Sigma^*$ where $\Sigma=I \times O$ is  monitorable iff:
\begin{itemize}
	\item there exists a monitor $M$ for $\varphi$, and
	\item there exists a word $\sigma\in \Sigma^*$, such that monitor $M$ provides a conclusive verdict for $\sigma$.	
\end{itemize}
\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\red{
We will define monitor with three cases, (i.e., verdict given by the monitor belongs to the set $\{true, false, unkonwn\}$).
The monitor returns $true$ when the current observation followed by any extension of it satisfies $\varphi$ (where $\varphi$ defines minimality property.)
It returns $false$ when the current observation followed by any extension of it satisfies $\neg\varphi$, where $\neg\varphi$ is negation of $\varphi$ (defined  as non-minimality). It returns $unknown$ for the current observation if the above two cases do not hold. 
}


\red{
Note that monitorability of a property depends on the size of the set of possible inputs $|I|$.
If the set of possible inputs is bounded, then the property is monitorable. 
Note that the set of possible inputs $I$ is finite. 
Let $|I| =n$, then there certainly exists a word $\sigma \in \Sigma^*$ of length $n$, where every input $i\in I$ appears (only) once in $\sigma$. 
Let $\cal{F}: I \rightarrow O$ be the functional program that we want to check for satisfaction (violation) of data minimality.
Instead of monitoring behavior of $\cal{F}$ at runtime (where inputs observed by the monitor may be repeated), let us consider that we want to test $\cal{F}$ for minimality using monitoring (where we have control over the inputs that can be considered in future iterations).
}  

%%%


\remove{
\red{Note that the monitoring mechanism that we define can be used also after deployment. In this case, we cannot give a bound on the length of the input observation, maximum input-output events to be observed to give a conclusive verdict.}
}

==> content/relatedWork.tex <==
%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:rw}
%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Runtime verification.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Runtime verification mechanisms for trace properties has been extensively studied and several RV frameworks have been proposed such as \cite{Havelund2008,Bauer:2011:RVL,Blech2012}.
RV approaches focus on the synthesis of a verification monitor from a given property, and the system being monitored is considered to be a black-box.
Properties are usually specified in high-level formalisms with a semantics customised for finite executions such as automata~\cite{FalconeFM09} or some variant of Linear Temporal Logic (LTL) such as LTL$_3$~\cite{Bauer:2011:RVL} or RV-LTL~\cite{BauerLS10}.
%For a short survey and tutorial on runtime verification techniques, see~\cite{LeuckerS08jlap,FalconeHR13}.
For instance, in~\cite{Bauer:2011:RVL} monitors are automatically synthesized from properties defined using a variant of LTL.
The monitor synthesis approach in~\cite{Bauer:2011:RVL} involves building an automaton that accepts a given LTL property (property $\varphi$ to be monitored), and an automaton that accepts negation of $\varphi$, and testing emptiness from the states reached in both these automata upon the current observed input word.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Runtime verification of hyper-properties.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



